Field of Junctions: Extracting Boundary Structure at Low SNR

We introduce a bottom-up model for simultaneously finding many boundary elements in an image, including contours, corners and junctions. The model explains boundary shape in each small patch using a 'generalized M-junction' comprising M angles and a freely-moving vertex. Images are analyzed using non-convex optimization to cooperatively find M+2 junction values at every location, with spatial consistency being enforced by a novel regularizer that reduces curvature while preserving corners and junctions. The resulting 'field of junctions' is simultaneously a contour detector, corner/junction detector, and boundary-aware smoothing of regional appearance. Notably, its unified analysis of contours, corners, junctions and uniform regions allows it to succeed at high noise levels, where other methods for segmentation and boundary detection fail.

==> sections/increasing_noise.tex <==
\newpage



\section{Additional comparisons with increasing noise}

Figure~\ref{figure:fig2} provides an extended comparison of our method to previous methods, similar to Figure~2 from the main paper. Here we gradually increase the noise level of the input image, showing the noise level at which each existing method breaks.


\begin{figure}[H]
\begin{minipage}{0.25\textwidth}
\vbox to \figtwospace {\vfil \null\hfill Input \qquad\qquad \vfil}
\vbox to \figtwospace {\vfil \null\hfill HED \qquad\qquad\vfil}
\vbox to \figtwospace {\vfil \null\hfill Canny \qquad\qquad\vfil}
\vbox to \figtwospace {\vfil \null\hfill gPb \qquad\qquad\vfil}
\vbox to \figtwospace {\vfil \null\hfill ORB \qquad\qquad\vfil}
\vbox to \figtwospace {\vfil \null\hfill ASJ \qquad\qquad\vfil}
\vbox to \figtwospace {\vfil \null\hfill GrabCut \qquad\qquad\vfil}
\vbox to \figtwospace {\vfil \null\hfill Chan-Vese \qquad\qquad\vfil}
\vbox to \figtwospace {\vfil \null\hfill $\text{L}_0$ \qquad\qquad\vfil}
\vbox to \doublefigtwospace {\vfil \null\hfill Field of Junctions \quad\, $\left[\rule{0cm}{\figtwobracket}\right.$ \vfil}
\vbox to 0pt {\vfil\vfil}
\end{minipage} %\hfill
\begin{minipage}{0.6\textwidth}
\includegraphics[width=\linewidth]{figures/fig1_big.png}
\end{minipage}
\caption{\label{figure:fig2} Analyzing the same image at multiple noise levels. From top to bottom: input image, boundary maps from edge detectors (HED, Canny, gPb); detections of corners or junctions superimposed on the input (ORB, ASJ); binary segmentations using manual initialization shown with thin lines (GrabCut, Chan-Vese) or without manual initialization ($\text{L}_0$); and output from the field of junctions. Existing approaches fail in the high noise regime, but the field of junctions does not.}
\end{figure}


\newpage

Figure~\ref{figure:fig2_SIDD} provides a comparison of our method to previous methods on patches from the Smartphone Image Denoising Dataset (SIDD)~\cite{abdelhamed2018high} captured at decreasing light levels.

\begin{figure}[H]
\begin{minipage}{0.25\textwidth}
\vbox to \figtwosiddspace {\vfil \null\hfill Input \qquad\qquad \vfil}
\vbox to \figtwosiddspace {\vfil \null\hfill HED \qquad\qquad\vfil}
\vbox to \figtwosiddspace {\vfil \null\hfill Canny \qquad\qquad\vfil}
\vbox to \figtwosiddspace {\vfil \null\hfill gPb \qquad\qquad\vfil}
\vbox to \figtwosiddspace {\vfil \null\hfill ORB \qquad\qquad\vfil}
\vbox to \figtwosiddspace {\vfil \null\hfill ASJ \qquad\qquad\vfil}
\vbox to \figtwosiddspace {\vfil \null\hfill GrabCut \qquad\qquad\vfil}
\vbox to \figtwosiddspace {\vfil \null\hfill Chan-Vese \qquad\qquad\vfil}
\vbox to \figtwosiddspace {\vfil \null\hfill $\text{L}_0$ \qquad\qquad\vfil}
\vbox to \doublefigtwosiddspace {\vfil \null\hfill Field of Junctions \quad\, $\left[\rule{0cm}{\figtwosiddbracket}\right.$ \vfil}
\vbox to 0pt {\vfil\vfil}
\end{minipage} %\hfill
\begin{minipage}{0.7\textwidth}
\includegraphics[width=\linewidth]{figures/fig1_SIDD_low_contrast_points.png}
\end{minipage}
\caption{\label{figure:fig2_SIDD} Analyzing the same scene at multiple light levels. Images are taken from SIDD. (The images are displayed at lower contrast in the rows corresponding to ORB and ASJ for clarity.)}
\end{figure}

